Access Probability Optimization in RACH: A Multi-Armed Bandits Approach

The use of cellular networks for massive machine-type communications (mMTC) is an appealing solution due to the availability of the existing infrastructure. However, the massive number of user equipments (UEs) poses a significant challenge to the cellular network's random access channel (RACH) regarding congestion and overloading. To mitigate this problem, we first present a novel approach to model a two-priority RACH, which allows us to define access patterns that describe the random access behavior of UEs as observed by the base station (BS). A non-uniform preamble selection scheme is proposed, offering increased flexibility in resource allocation for different UE priority classes. Then, we formulate an allocation model that finds the optimal access probabilities to maximize the success rate of high-priority UEs while constraining low-priority UEs. Finally, we develop a reinforcement learning approach to solving the optimization problem using multi-armed bandits, which provides a near-optimal but scalable solution and does not require the BS to know the number of UEs in the network.

==> Acronyms.tex <==

\usepackage[acronym, toc]{glossaries}
\newacronym{RB}{RB}{resource block} 
\newacronym{IoT}{IoT}{Internet of things}
\newacronym{MTC}{MTC}{machine-type communication}
\newacronym{mMTC}{mMTC}{massive machine-type communication}
\newacronym{IIoT}{IIoT}{industrial Internet of Things}
\newacronym{HTC}{HTC}{Human-type communication}
\newacronym{MA}{MA}{multiple access}
\newacronym{PA}{PA}{priority access}
\newacronym{RACH}{RACH}{random access channel}
\newacronym{PRACH}{PRACH}{pysical random access channel}

\newacronym{PG}{PG}{power grid}
\newacronym[\glslongpluralkey={smart grids}, \glsshortpluralkey={SGs}]{SG}{SG}{smart grid} %
\newacronym{DOE}{DOE}{Department of Energy}
\newacronym{AMI}{AMI}{advanced metering infrastructure}
\newacronym{SM}{SM}{smart meter}
\newacronym{HAN}{HAN}{home area network}
\newacronym{DR}{DR}{demand response}
\newacronym{EV}{EV}{electric vehicle}
\newacronym{WASA}{WASA}{wide-area situational awareness}
\newacronym{DER}{DER}{distributed energy resources}
\newacronym{DGM}{DGM}{distributed energy management}
\newacronym{NIST}{NIST}{National Institute of Standards and Technology}
\newacronym{FERC}{FERC}{Federal Energy Regulatory Commission}

\newacronym{UE}{UE}{user equipment}
\newacronym{CB-MA}{CB-MA}{contention-based multiple access}
\newacronym{CF-MA}{CF-MA}{conflict-free multiple access}
\newacronym{FDMA}{FDMA}{frequency division multiple access}
\newacronym{TDMA}{TDMA}{time division multiple access}
\newacronym{CDMA}{CDMA}{code division multiple access}
\newacronym{SDMA}{OMA}{spatial division multiple access}
\newacronym{LDS-CDMA}{LDS-CDMA}{low density signature code division multiple access}
\newacronym{PDMA}{PDMA}{pattern division multiple access}
\newacronym{MUSA}{MUSA}{multi-user shared access}
\newacronym{SCMA}{SCMA}{sparce code multiple access}
\newacronym{IDMA}{IDMA}{interleave division multiple access}
\newacronym{SPMA}{SPMA}{statistical based multiple access}
\newacronym{DS-CDMA}{DS-CDMA}{direct sequence code division multiple access}
\newacronym{FH-CDMA}{FH-CDMA}{frequency hopping code division multiple access}

\newacronym{OMA}{OMA}{orthogonal multiple access}
\newacronym{NOMA}{NOMA}{non-orthogonal multiple access}
\newacronym{CD-NOMA}{CD-NOMA}{code domain non-orthogonal multiple access}
\newacronym{PD-NOMA}{PD-NOMA}{power domain non-orthogonal multiple access}
\newacronym{MIMO}{MIMO}{multiple input multiple output}
\newacronym{QAM}{QAM}{quadrature amplitude modulation}
\newacronym{FEC}{FEC}{forward error correction}
\newacronym{MAC}{MAC}{medium access control}
\newacronym{SIC}{SIC}{successive interference cancellation}
\newacronym{BS}{BS}{base station}
\newacronym{LTE}{LTE}{long-term evolution}
\newacronym{LTE-A}{LTE-A}{long-term evolution advanced}

\newacronym{SE}{SE}{spectral efficiency}
\newacronym{CSI}{CSI}{channel state information}
\newacronym{SUD}{SUD}{single-user detection}
\newacronym{MUD}{MUD}{multi-user detection}
\newacronym{MAP}{MAP}{maximum \textit{a posteriori}}
\newacronym{ML}{ML}{maximum likelihood}
\newacronym{RCML}{RCML}{reduced complexity maximum likelihood}
\newacronym{i.i.d.}{i.i.d.}{independent and identically distributed}

\newacronym{FDD}{FDD}{frequency division duplexing}
\newacronym{TDD}{TDD}{time division duplexing}
\newacronym{PSD}{PSD}{power spectral density}
\newacronym{MAI}{MAI}{multiple access interference}
\newacronym{QoS}{QoS}{quality of service}
\newacronym{TTNT}{TTNT}{Tactical Targeting Network Technology}
\newacronym{COS}{COS}{channel occupancy statistic}
\newacronym{PPP}{PPP}{Poisson point process}
\newacronym{3GPP}{3GPP}{3rd Generation Partnership Project}

\newacronym{H-UE}{H-UE}{high-priority user equipment}
\newacronym{L-UE}{L-UE}{low-priority user equipment}
\newacronym{ACB}{ACB}{access class barring}
\newacronym{D-ACB}{D-ACB}{dynamic access class barring}

\newacronym{QPAC}{QPAC}{queue-aware priority access classification}
\newacronym{PRADA}{PRADA}{prioritized random access with dynamic access barring}

\newacronym{RHS}{RHS}{right hand side}
\newacronym{LHS}{LHS}{left hand side}
\newacronym{MAE}{MAE}{mean absolute error}
\newacronym{SQP}{SQP}{sequential quadratic programming}

\newacronym{RL}{RL}{reinforcement learning}
\newacronym{MDP}{MDP}{Markov decision process}
\newacronym{MAB}{MAB}{multi-armed bandit}
\newacronym{UCB}{UCB}{upper confidence bound}
\newacronym{AS}{AS}{action space}
\newacronym{CAS}{CAS}{modified \gls{AS}}
\newacronym{e-greedy}{$\epsilon$-greedy}{epsilon-greedy}
\newacronym{DEG}{DEG}{decaying epsilon-greedy}
\newacronym{DQN}{DQN}{deep Q-network}
\newacronym[\glsshortpluralkey={algs.}]{alg}{alg.}{algorithm}
\newacronym{CE}{CE}{cross entropy}
\newacronym{PPO}{PPO}{proximal policy optimization}


